Deep Soft Procrustes for Markerless Volumetric Sensor Alignment

With the advent of consumer grade depth sensors, low-cost volumetric capture systems are easier to deploy. Their wider adoption though depends on their usability and by extension on the practicality of spatially aligning multiple sensors. Most existing alignment approaches employ visual patterns, e.g. checkerboards, or markers and require high user involvement and technical knowledge. More user-friendly and easier-to-use approaches rely on markerless methods that exploit geometric patterns of a physical structure. However, current SoA approaches are bounded by restrictions in the placement and the number of sensors. In this work, we improve markerless data-driven correspondence estimation to achieve more robust and flexible multi-sensor spatial alignment. In particular, we incorporate geometric constraints in an end-to-end manner into a typical segmentation based model and bridge the intermediate dense classification task with the targeted pose estimation one. This is accomplished by a soft, differentiable procrustes analysis that regularizes the segmentation and achieves higher extrinsic calibration performance in expanded sensor placement configurations, while being unrestricted by the number of sensors of the volumetric capture system. Our model is experimentally shown to achieve similar results with marker-based methods and outperform the markerless ones, while also being robust to the pose variations of the calibration structure. Code and pretrained models are available at https://vcl3d.github.io/StructureNet/.

==> SoftAttention.tex <==
\begin{figure*}
\begin{center}
   \includegraphics[width=\linewidth]{figures/merged.png}
\end{center}
   \vspace{-0.2in}
   \caption{Virtual representations of setups on which methods were evaluated. In more detail, please refer to section \ref{sec:results}. From left to right: (\textbf{a}) shows the \textit{array configuration} used to capture real data for comparison as described in \ref{sec:self_evaluation}; (\textbf{b}) showcases the \textit{arc configuration}; and (\textbf{c}) shows a full 360 setup with alternating camera heights. 
   Both (\textbf{b}) and (\textbf{c}) used for calibration setup evaluation and comparison against other methods, further described in \ref{sec:comparisson_other_methods}.}
\label{fig:test_samples}
\vspace{-0.2in}
\end{figure*}

Our autoencoder, depicted in Fig.~\ref{fig:net}, consists of 3 parts, namely an encoder, a bottleneck part, and a decoder. 
The encoder consists of 14 convolutional layers (CONV) each one followed by a Rectified Linear Unit (ReLU) that thresholds the activations. 
The input depthmap is downsampled 4 times using max pooling operators (POOL). 
The output of the encoder is further processed by the bottleneck part, which consists of 4 residual blocks, each following a ReLU-CONV-ReLU-CONV structure, adopting the identity mapping with pre-activation originally proposed in~\cite{he} for performance improvement. 
The decoder shares similar structure with the encoder, using 14 CONV followed by ReLU non-linearities. 
Note that the input feature map is upsampled 4 times prior to the segmentation prediction, using nearest neighbor interpolation. 
A $softmax$ function follows, which is applied at each pixel of the decoder output and serves as the initial estimation of the visible sides of each box. 
Finally, following the U-Net structure proposed in~\cite{ronn}, we use skip connections to additionally propagate the activations of specific encoder layers with the corresponding ones of the decoder. 
We train our model by jointly rendering synthetic views and label maps of the virtual model in a variety of poses. In particular, we minimize a total loss that is realised as:
\begin{equation}
    \pazocal{L}_{total} = \pazocal{L}_{seg} + \lambda \pazocal{L}_{3D},
\end{equation}
where $\pazocal{L}_{seg}$ is the per pixel negative log-likelihood of the predicted and ground truth planar visible side labels, normalized over the total number of pixels, $\pazocal{L}_{3D}$ is the 3D keypoint correspondence defined in Eq.~\ref{eq:loss_function}, and $\lambda$ is a regularization term that controls the contribution of $\pazocal{L}_{3D}$ to the total loss.

In order to achieve faster convergence and improve the performance of our autoencoder, we introduce a soft-attention mechanism that forces the model to implicitly focus at the calibration structure. 
The mechanism that can be visualized in Fig.~\ref{fig:net}, is placed between the bottleneck part and the decoder of the model. 
In particular, given the activation matrix of the last residual block ${A} \in \mathbb{R}^{d\times h\times w}$, where $d$ is the number of channels of the activation map, we use a separate branch to convolve $A$ with a kernel of $1\times 1$ size, and apply a $sigmoid$ function to normalize the activation values to the $[0,1]$ space, thus forming an excitation mask $M \in [0,1]^{h\times w}$.
Note, that $M$ is multiplied with $A$ in an element-wise manner and then upsampled and re-applied to the activation maps after each upsampling layer of the decoder.
